End-to-End Feasible Optimization Proxies for Large-Scale Economic Dispatch

The paper proposes a novel End-to-End Learning and Repair (E2ELR) architecture for training optimization proxies for economic dispatch problems. E2ELR combines deep neural networks with closed-form, differentiable repair layers, thereby integrating learning and feasibility in an end-to-end fashion. E2ELR is also trained with self-supervised learning, removing the need for labeled data and the solving of numerous optimization problems offline. E2ELR is evaluated on industry-size power grids with tens of thousands of buses using an economic dispatch that co-optimizes energy and reserves. The results demonstrate that the self-supervised E2ELR achieves state-of-the-art performance, with optimality gaps that outperform other baselines by at least an order of magnitude.

==> tables/hyperparameters_DCOPF-R.tex <==
\begin{tabular}{llrrrr}
\toprule
\multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{System} & \multicolumn{1}{c}{Model} &  \multicolumn{1}{c}{$\lambda$} & \multicolumn{1}{c}{$l$} & \multicolumn{1}{c}{$hd$} \\
\midrule
SL & \ieeeSmall & DNN & $10^{-4}$ & 3 & 128 \\
 & \ieeeSmall & E2ELR & $10^{-4}$ & 3 & 256 \\
 & \ieeeSmall & DC3 & $10^{-5}$ & 4 & 256 \\
 & \pegaseSmall & DNN & $10^{-6}$ & 3 & 256 \\
 & \pegaseSmall & E2ELR & $10^{-6}$ & 3 & 128 \\
 & \pegaseSmall & DC3 & $10^{-6}$ & 3 & 256 \\
 & \rteLarge & DNN & $10^{-4}$ & 3 & 256 \\
 & \rteLarge & E2ELR & $10^{-6}$ & 3 & 256 \\
 & \rteLarge & DC3 & $10^{-6}$ & 3 & 256 \\
 & \pegaseLarge & DNN & $10^{-5}$ & 3 & 256 \\
 & \pegaseLarge & E2ELR & $10^{-6}$ & 3 & 256 \\
 & \pegaseLarge & DC3 & $10^{-6}$ & 3 & 256 \\
 & \pegaseXLarge & DNN & $10^{-5}$ & 3 & 256 \\
 & \pegaseXLarge & E2ELR & $10^{-6}$ & 4 & 256 \\
 & \pegaseXLarge & DC3 & $10^{-6}$ & 3 & 256 \\
 & \gocXXL & DNN & $10^{-6}$ & 3 & 128 \\
 & \gocXXL & E2ELR & $10^{-6}$ & 4 & 256 \\
 & \gocXXL & DC3 & $10^{-6}$ & 3 & 256 \\
\midrule
SSL 
 & \ieeeSmall & DNN & $10^{-1}$ & 3 & 256 \\
 & \ieeeSmall & E2ELR & - & 3 & 256 \\
 & \ieeeSmall & DC3 & $10^{-1}$ & 3 & 256 \\
 & \pegaseSmall & DNN & $10^{-1}$ & 3 & 128 \\
 & \pegaseSmall & E2ELR & - & 3 & 256 \\
 & \pegaseSmall & DC3 & $10^{-1}$ & 4 & 128 \\
 & \rteLarge & DNN & $10^{-0}$ & 3 & 128 \\
 & \rteLarge & E2ELR & - & 3 & 256 \\
 & \rteLarge & DC3 & $10^{-0}$ & 4 & 256 \\
 & \pegaseLarge & DNN & $10^{-1}$ & 4 & 256 \\
 & \pegaseLarge & E2ELR & - & 3 & 256 \\
 & \pegaseLarge & DC3 & $10^{-1}$ & 3 & 256 \\
 & \pegaseXLarge & DNN & $10^{-1}$ & 4 & 256 \\
 & \pegaseXLarge & E2ELR & - & 3 & 128 \\
 & \pegaseXLarge & DC3 & $10^{-1}$ & 3 & 256 \\
 & \gocXXL & DNN & $10^{-1}$ & 3 & 128 \\
 & \gocXXL & E2ELR & - & 4 & 256 \\
 & \gocXXL & DC3 & $10^{-1}$ & 3 & 256 \\
\bottomrule
\end{tabular}

==> tables/hyperparameters_DCOPF.tex <==
\begin{tabular}{lllrrr}
\toprule
\multicolumn{1}{c}{Loss} & \multicolumn{1}{c}{System} & \multicolumn{1}{c}{Model} & \multicolumn{1}{c}{$\lambda$} & \multicolumn{1}{c}{$l$} & \multicolumn{1}{c}{$hd$} \\
\midrule
SL & \ieeeSmall & DNN & $10^{-4}$ & 3 & 256 \\
 & \ieeeSmall & E2ELR & $10^{-4}$ & 4 & 256 \\
 & \ieeeSmall & DC3 & $10^{-5}$ & 4 & 256 \\
 & \ieeeSmall & LOOP & $10^{-4}$ & 4 & 128 \\
 & \pegaseSmall & DNN & $10^{-6}$ & 3 & 128 \\
 & \pegaseSmall & E2ELR & $10^{-6}$ & 4 & 256 \\
 & \pegaseSmall & DC3 & $10^{-6}$ & 4 & 128 \\
 & \pegaseSmall & LOOP & $10^{-5}$ & 3 & 256 \\
 & \rteLarge & DNN & $10^{-6}$ & 3 & 256 \\
 & \rteLarge & E2ELR & $10^{-6}$ & 3 & 256 \\
 & \rteLarge & DC3 & $10^{-6}$ & 3 & 256 \\
 & \rteLarge & LOOP & $10^{-5}$ & 4 & 128 \\
 & \pegaseLarge & DNN & $10^{-6}$ & 4 & 256 \\
 & \pegaseLarge & E2ELR & $10^{-6}$ & 4 & 256 \\
 & \pegaseLarge & DC3 & $10^{-6}$ & 4 & 256 \\
 & \pegaseLarge & LOOP & $10^{-5}$ & 3 & 256 \\
 & \pegaseXLarge & DNN & $10^{-6}$ & 3 & 256 \\
 & \pegaseXLarge & E2ELR & $10^{-6}$ & 3 & 128 \\
 & \pegaseXLarge & DC3 & $10^{-6}$ & 3 & 256 \\
 & \pegaseXLarge & LOOP & $10^{-5}$ & 3 & 128 \\
 & \gocXXL & DNN & $10^{-5}$ & 4 & 128 \\
 & \gocXXL & E2ELR & $10^{-6}$ & 3 & 128 \\
 & \gocXXL & DC3 & $10^{-6}$ & 3 & 256 \\
 & \gocXXL & LOOP & $10^{-5}$ & 3 & 128 \\
\midrule
SSL 
 & \ieeeSmall & DNN & $10^{-1}$ & 3 & 256 \\
 & \ieeeSmall & E2ELR & - & 3 & 256 \\
 & \ieeeSmall & DC3 & $10^{-1}$ & 3 & 256 \\
 & \ieeeSmall & LOOP & - & 3 & 256 \\
 & \pegaseSmall & DNN & $10^{-1}$ & 3 & 256 \\
 & \pegaseSmall & E2ELR & - & 4 & 256 \\
 & \pegaseSmall & DC3 & $10^{-1}$ & 4 & 128 \\
 & \pegaseSmall & LOOP & - & 3 & 256 \\
 & \rteLarge & DNN & $10^{-0}$ & 3 & 128 \\
 & \rteLarge & E2ELR & - & 3 & 256 \\
 & \rteLarge & DC3 & $10^{-1}$ & 4 & 256 \\
 & \rteLarge & LOOP & - & 4 & 128 \\
 & \pegaseLarge & DNN & $10^{-1}$ & 4 & 256 \\
 & \pegaseLarge & E2ELR & - & 3 & 256 \\
 & \pegaseLarge & DC3 & $10^{-1}$ & 4 & 256 \\
 & \pegaseLarge & LOOP & - & 3 & 128 \\
 & \pegaseXLarge & DNN & $10^{-1}$ & 3 & 256 \\
 & \pegaseXLarge & E2ELR & - & 4 & 128 \\
 & \pegaseXLarge & DC3 & $10^{-1}$ & 3 & 256 \\
 & \pegaseXLarge & LOOP & - & 3 & 128 \\
 & \gocXXL & DNN & $10^{-1}$ & 4 & 256 \\
 & \gocXXL & E2ELR & - & 4 & 256 \\
 & \gocXXL & DC3 & $10^{-1}$ & 4 & 256 \\
 & \gocXXL & LOOP & - & 4 & 128 \\
\bottomrule
\end{tabular}
